Calibration of mid- to far-infrared spectral lines in galaxies

Mid- to far-infrared (IR) lines are suited to study dust obscured regions in galaxies, because IR spectroscopy allows us to explore the most hidden regions where heavily obscured star formation as well as accretion onto supermassive black-holes occur. This is mostly important at redshifts of 1<z<3, when most of the baryonic mass in galaxies has been assembled. We provide reliable calibrations of the mid- to far-IR ionic fine structure lines, the brightest H2 pure rotational lines and the Polycyclic Aromatic Hydrocarbons (PAHs) features, that will be used to analyse current and future observations in the mm/submm range from the ground, as well as mid-IR spectroscopy from the upcoming James Webb Space Telescope. We use three samples of galaxies observed in the local Universe: star forming galaxies, AGN and low-metallicity dwarf galaxies. For each population we derive different calibrations of the observed line luminosities versus the total IR luminosities. We derive spectroscopic measurements of SFR and BHAR using mid- and far-IR fine structure lines, H2 pure rotational lines and PAH features. We derive robust star-formation tracers based on the [CII]158 $\mu$m line; the sum of the [OI]63$\mu$m and [OIII]88$\mu$m lines; a combination of the neon and sulfur mid-IR lines; the bright PAH features at 6.2 and 11.3 $\mu$m, and the H2 rotational lines at 9.7, 12.3 and 17 $\mu$m. We propose the [CII]158$\mu$m line, the combination of two neon lines and, for solar-like metallicity galaxies that may harbor an AGN, the PAH11.3$\mu$m feature as the best SFR tracers. A reliable measure of the BHAR can be obtained using the [OIV]25.9 $\mu$m and the [NeV]14.3 and 24.3 $\mu$m lines. For the most commonly observed fine-structure lines in the far-IR we compare our calibration with the existing ALMA observations of high redshift galaxies finding overall a good agreement with local results.

==> line_specifications.tex <==
\afterpage{%
\begin{landscape}
\begin{table}
%\tabletypesize{\footnotesize}
%\setlength{\tabcolsep}{0.3em}
%\tablecolumns{11} 
%\tablewidth{0pt}
\caption{Fine-structure lines in the mid- to far-IR range. The columns correspond to the central wavelength, frequency, ionisation potential, excitation temperature, critical density, spectral and spatial resolution of the data presented in this work, and the number of AGN, starburst, and dwarfs galaxies with line detections above $3 \times$\,\textsc{rms}. Critical densities and excitation temperatures from: \citet{launay1977,tielens1985,greenhouse1993,sturm2002,cormier2012,farrah2013}.}\label{tbl_lines}

\begin{threeparttable}[b]
\begin{tabular}{lcccccccccc}
\bf Line & \bf $\lambda$ & \bf $\nu$ & \bf I.P. & \bf E & \bf $n_{\rm cr}$ & \bf Spec. Res. & \bf Ang. Res.
  & ($\mu$m)                   & (GHz)                    & (eV) & (K) & ($\rm{cm^{-3}}$) &($\rm{km\,s^{-1}}$)                        & (arcsec)  
\hline \\[-0.3cm]
\nevi$^2$P$_{3/2}$--$^2$P$_{1/2}$    & 7.65   & 39188.56 & 126.21 & 1888 & $2.5 \times 10^5$           & $\sim 1500$  & $14 \times 20$     \\
\ariii $^3$P$_2$--$^3$P$_1$          & 8.99   & 3334.73  & 27.36  & 1600 & $3.1 \times 10^{5}$         & $\sim 1500$  & $14 \times 20$     \\
H$_2$ (0,0) S(3)                     & 9.66   & 31034.41 & 4.48   & 2504 & $9 \times 10^{5}$\tnote{a}  & $\sim 500$   & $4.7 \times 11.3$  \\
\siv$^2$P$_{3/2}$--$^2$P$_{1/2}$     & 10.51  & 28524.50 & 34.79  & 1369 & $5.39 \times 10^4$          & $\sim 500$   & $4.7 \times 11.3$  \\
H$_2$ (0,0) S(2)                     & 12.28  & 24413.07 & 4.48   & 1682 & $2 \times 10^{5}$\tnote{a}  & $\sim 500$   & $4.7 \times 11.3$  \\
\neii$^2$P$_{1/2}$--$^2$P$_{3/2}$    & 12.81  & 23403.00 & 21.56  & 1123 & $7.00 \times 10^5$          & $\sim 500$   & $4.7 \times 11.3$  \\
\nev$^3$P$_2$--$^3$P$_1$             & 14.32  & 20935.23 & 97.12  & 1892 & $3 \times 10^4$             & $\sim 500$   & $4.7 \times 11.3$  \\
\clii $^3$P$_2$--$^3$P$_1$           & 14.37  & 2086.23  & 12.97  & 1001 & --                          & $\sim 500$   & $4.7 \times 11.3$  \\
\neiii$^3$P$_1$--$^3$P$_2$           & 15.55  & 19266.87 & 40.96  & 925  & $2.68 \times 10^5$          & $\sim 500$   & $4.7 \times 11.3$  \\
H$_2$ (0,0) S(1)                     & 17.03  & 17603.78 & 4.48   & 1015 & $2 \times 10^{4}$\tnote{a}  & $\sim 500$   & $4.7 \times 11.3$  \\
\feii a$^4$F$_{7/2}$--a$^4$F$_{9/2}$ & 17.93  & 16720.16 & 7.90   & 802  &  --                         & $\sim 500$   & $4.7 \times 11.3$  \\
\siii$^3$P$_2$--$^3$P$_1$            & 18.71  & 16023.11 & 23.34  & 769  & $2.22 \times 10^4$          & $\sim 500$   & $4.7 \times 11.3$  \\
\feiii $^5$D$_4$--$^5$D$_3$          & 22.93  & 13074.24 & 16.19  & 627  & $ 10^{5}$                   & $\sim 500$   & $4.7 \times 11.3$  \\
\nev$^3$P$_1$--$^3$P$_0$             & 24.32  & 12326.99 & 97.12  & 596  & $5.0 \times 10^5$           & $\sim 500$   & $11.1 \times 22.3$ \\
\oiv$^2$P$_{3/2}$--$^2$P$_{1/2}$     & 25.89  & 11579.47 & 54.94  & 555  & $10^4$                      & $\sim 500$   & $11.1 \times 22.3$ \\
\feii a$^6$D$_{7/2}$--a$^6$D$_{9/2}$ & 25.98  & 11539.35 & 7.9    & 553  & $2.2 \times 10^6$           & $\sim 500$   & $11.1 \times 22.3$ \\
H$_2$ (0,0) S(0)                     & 28.22  & 10380.62 & 4.48   & 510  & $7 \times 10^{2}$\tnote{a}  & $\sim 500$   & $11.1 \times 22.3$ \\
\siii$^3$P$_1$--$^3$P$_0$            & 33.48  & 8954.37  & 23.34  & 430  & $7.04 \times 10^3$          & $\sim 500$   & $11.1 \times 22.3$ \\
\sitwo$^2$P$_{3/2}$--$^2$P$_{1/2}$   & 34.81  & 8612.25  & 8.15   & 413  & $3.4 \times 10^5$\tnote{a},$10^3$ & $\sim 500$ & $11.1 \times 22.3$  \\
\oiii$^3$P$_2$--$^3$P$_1$            & 51.81  & 5787.57  & 35.12  & 441  & $3.6 \times 10^3$           & $\sim 105$   & 9.4\tnote{b}\\
\niii$^2$P$_{3/2}$--$^2$P$_{1/2}$    & 57.32  & 5230.43  & 29.60  & 251  & $3.0 \times 10^3$           & $\sim 105$   & 9.4 &  \\ 
\oi$^3$P$_2$--$^3$P$_1$              & 63.18  & 4744.77  & --     & 228  & $4.7 \times 10^5$\tnote{a}  & $\sim 86$    & 9.4 &  \\ 
\oiii$^3$P$_1$--$^3$P$_0$            & 88.36  & 3393.01  & 35.12  & 163  & $510$                       & $\sim 124$   & 9.4  \\
\nii$^3$P$_2$--$^3$P$_1$             & 121.90 & 2459.38  & 14.53  & 118  & $310$                       & $\sim 290$   & 9.4 \\
\oi$^3$P$_1$--$^3$P$_0$              & 145.52 & 2060.07  & --     & 98   & $9.5 \times 10^4$\tnote{a}  & $\sim 256$   & 10.3 \\
\cii$^2$P$_{3/2}$--$^2$P$_{1/2}$     & 157.74 & 1900.54  & 11.26  & 91   & $50$,$2.8 \times 10^3$\tnote{a} & $\sim 238$  & 11.2 \\
\nii$^3$P$_1$--$^3$P$_0$             & 205.3  & 1460.27  & 14.53  & 70   & $48$                         & $\sim 297$  & $\sim16.8$\\
\ci$^3$P$_{2}$--$^3$P$_{1}$          & 370.37 & 809.44   & --     & 38.9 & $2.8 \times 10^{3}$\tnote{a} & $\sim 536$  & $\sim 35.0$  \\
\ci$^3$P$_{1}$--$^3$P$_{0}$          & 609.7  & 491.70   & --     & 23.6 & $4.7 \times 10^{2}$\tnote{a} & $\sim 882$  & $\sim 35.0$       \\
\hline

\end{tabular}
\begin{tablenotes}
    \item[a] Critical density for collisions with hydrogen atoms.
    \item[b] The beam size for \textit{Herschel}/PACS is dominated by the spaxel size ($9\farcs4$) below $\sim 120\, \rm{\micron}$.
\end{tablenotes}
\end{threeparttable}
\end{table}
\end{landscape}}
